Automated Linear Parameter-Varying Modeling of Nonlinear Systems: A Global Embedding Approach

In this paper, an automated Linear Parameter-Varying (LPV) model conversion approach is proposed for nonlinear dynamical systems. The proposed method achieves global embedding of the original nonlinear behavior of the system by leveraging the second fundamental theorem of calculus to factorize matrix function expressions without any approximation. The implementation of the proposed method in the LPVcore toolbox for Matlab is discussed, and its performance is showcased on a comprehensive example of automated LPV model conversion of an unbalanced disk system, which is then used to design an LPV controller that is deployed on the original nonlinear system. In addition, the conversion capabilities are further demonstrated by obtaining an LPV embedding of a three-degree-of-freedom control moment gyroscope. All software implementations are available at www.lpvcore.net.

==> chapters/ftcRoland.tex <==
\section{FTC embedding from paper Roland sent}

The core idea is that if given a continuously differentiable function $g:\mathbb{R}^n\rightarrow\mathbb{R}^m$, then based on the FTC~\cite{Koelewijn2023}:
Let us assume we have a continuously differentiable function $g:\mathbb{R}^n\rightarrow\mathbb{R}^m$, with $g(0)=0$, for which we have that $g(\eta)=\begin{bmatrix}
		g_1(\eta) & \cdots & g_m(\eta)
	\end{bmatrix}$, where $g_i(\eta):\mathbb{R}^n\rightarrow\mathbb{R}$ for $ i = 1,\,\dots,\,m$ and $\eta\in\mathbb{R}^n$. Let us define the element\nobreakdash-wise functions $\bar{g}_i(\lambda)=g_i(\lambda \eta)$ for $i = 1,\,\dots,\,m$, with $\bar{g}_i:[0,1]\rightarrow\mathbb{R}$. Using the second fundamental theorem of calculus:
\begin{equation}
	\bar{g}_i(1)-\bar{g}_i(0)=\int_0^1 \frac{d \bar{g}_i}{d\lambda}(\bar{\lambda})\;d\bar{\lambda},\quad\text{for }i=1,\dots\,m,
\end{equation}
results in
\begin{align}
	g_i(\eta)-\underbrace{g_i(0)}_0 & =\int_0^1\left(\frac{d g_i}{d\eta}(\bar{\lambda}\eta)\right)\eta \;d\bar{\lambda}, \quad\text{for }i=1,\dots\,m, \\
	g_i(\eta)                       & =\left(\int_0^1\frac{d g_i}{d\eta}(\bar{\lambda}\eta)\,d\bar{\lambda}\right)\eta.
\end{align}
Combining the elements, $g$ is expressed as
\begin{subequations}
	\begin{align}
		g(\eta)- g(0) & =                                                                                                                        %\begin{bmatrix}
		%g_1(\eta)\\\vdots\\g_m(\eta)
		%\end{bmatrix} 
		{\small
		\begin{bmatrix}
			\left(\int_0^1\frac{d g_1}{d\eta}({\lambda}\eta)\,d{\lambda}\right)(\eta-0) \\\vdots\\\left(\int_0^1\frac{d g_m}{d\eta}({\lambda}\eta)\,d{\lambda}\right)(\eta-0)
		\end{bmatrix}} \\
		g(\eta)- g(0) & =\left(\int_0^1\frac{d g}{d\eta}({\lambda}\eta)\,d{\lambda}\right)\eta,
	\end{align}
\end{subequations}
where $\frac{d g}{d\eta}({\lambda}\eta) \in \mathbb{R}^{m \times n}$ is the Jacobian of $g$ evaluated in ${\lambda}\eta$. Provided that functions $f$ and $h$ in \eqref{eq:nl_dyn} are differentiable, choosing  $\eta=[\
	\hat{x}^\top \ \ u^\top \ ]^\top$ gives via the FTC that
%\begin{equation*}%\label{eq:abcd_def}
\begin{align}
	\tilde{f}_{\hat \theta}(\hat{x},u) & \!=\!\underbrace{  \left({\int_0^1\!\!\frac{\partial f}{\partial \hat{x}}({\lambda}\hat{x},{\lambda}u)\,d\lambda}\right)}_{{A}(\hat{x},u)}\!\hat{x}\!+\!\underbrace{\left(\int_0^1\!\!\frac{\partial f}{\partial u}({\lambda}\hat{x},{\lambda}u)\,d\lambda\right)}_{{B}(\hat{x},u)}\!u, \notag \\
	\tilde{h}_{\hat \theta}(\hat{x})   & \!=\!\underbrace{\left(\int_0^1\!\!\frac{\partial h}{\partial \hat{x}}({\lambda}\hat{x})\,d\lambda\right)}_{{C}(\hat{x})}\!\hat{x}, \label{eq:abcd_def}                                                                                                                                        %\!+\!\underbrace{\left(\int_0^1\!\!\frac{\partial h}{\partial u}({\lambda}\hat{x},{\lambda}u)\,d\lambda\right)}_{{D}(\hat{x},u)}\!u,
\end{align}
%\end{equation*}
\vskip -2mm \noindent where $	\tilde{f}_{\hat \theta}(\hat{x},u)=f_{\hat \theta}(\hat{x},u)-	f_{\hat \theta}(0,0)$ with $\tilde{h}_{\hat \theta}$ similarly defined. With $p_k=[\
	\hat{x}_k^\top \ \ u_k^\top \ ]^\top$ and $\mu$ the identity function, this gives an LPV form of the ANN-SS model \eqref{eq:model_structure} with affine terms $V=	f_{\hat \theta}(0,0)$ and  $W=	h_{\hat \theta}(0)$ as
\begin{subequations}
	\label{eq:lpv_model}\begin{align}
		\hat{x}_{k+1} & = A(p_k) \hat{x}_k + B(p_k)  u_k + V, \\
		y_k           & = C(p_k)\hat{x}_k                     %+ D(p_k)  u_k
		+ W.
	\end{align}
\end{subequations}
